Error Compensated Quantized SGD and its Applications to Large-scale Distributed Optimization

Large-scale distributed optimization is of great importance in various applications. For data-parallel based distributed learning, the inter-node gradient communication often becomes the performance bottleneck. In this paper, we propose the error compensated quantized stochastic gradient descent algorithm to improve the training efficiency. Local gradients are quantized to reduce the communication overhead, and accumulated quantization error is utilized to speed up the convergence. Furthermore, we present theoretical analysis on the convergence behaviour, and demonstrate its advantage over competitors. Extensive experiments indicate that our algorithm can compress gradients by a factor of up to two magnitudes without performance degradation.

==> figures/error_bound_comparison.tex <==
\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[trim={0 0 0.5in 0.5in}, clip, width=.8\columnwidth]{pics/error_bound_comparison}}
\caption{Comparison on the reduction ratio of $\tau^{( t - \Delta t )}$ for various $\Delta t$. Here we let $\alpha = 0.01$, $\beta = 1$, and $\eta a_{1} = 1e{-}4$.}
\label{fig:error_bound_comparison}
\end{center}
\end{figure}

==> figures/error_vs_comp_ratio.tex <==
\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{pics/error_vs_comp_ratio}}
\caption{Comparison on the classification error rate versus compression ratio of gradients for training ResNet-20 on CIFAR-10.}
\label{fig:error_vs_comp_ratio}
\end{center}
\end{figure}

==> tables/speed_resnet152_ilsvrc12.tex <==
\begin{table}[!ht]
\caption{Comparison on the run-time speed (unit: millisecond per mini-batch) for training ResNet-50 on ILSVRC-12.}
\label{tab:speed_resnet152_ilsvrc12}
\centering
\vskip 0.15in
\begin{small}
\begin{sc}
\begin{tabular}{cccc}
\toprule
\# of GPUs & 32Bit-FP & QSGD & Opt-QSGD \\
\midrule 
2 & 579.87 & 415.64 & 415.24 \\
4 & 676.68 & 462.51 & 458.51 \\
8 & 845.85 & 533.28 & 518.28 \\
16 & 1137.61 & 670.34 & 671.44 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\vskip -0.1in
\end{table}
